SADAS: A Dialogue Assistant System Towards Remediating Norm Violations in Bilingual Socio-Cultural Conversations

In today's globalized world, bridging the cultural divide is more critical than ever for forging meaningful connections. The Socially-Aware Dialogue Assistant System (SADAS) is our answer to this global challenge, and it's designed to ensure that conversations between individuals from diverse cultural backgrounds unfold with respect and understanding. Our system's novel architecture includes: (1) identifying the categories of norms present in the dialogue, (2) detecting potential norm violations, (3) evaluating the severity of these violations, (4) implementing targeted remedies to rectify the breaches, and (5) articulates the rationale behind these corrective actions. We employ a series of State-Of-The-Art (SOTA) techniques to build different modules, and conduct numerous experiments to select the most suitable backbone model for each of the modules. We also design a human preference experiment to validate the overall performance of the system. We will open-source our system (including source code, tools and applications), hoping to advance future research. A demo video of our system can be found at:~\url{https://youtu.be/JqetWkfsejk}. We have released our code and software at:~\url{https://github.com/AnonymousEACLDemo/SADAS}.

==> eacl2024-latex/2-background.tex <==
\section{Background}
%
In the realm of social interaction, norms are regarded as patterns of behavior that serve as guidelines for appropriate conduct in a given context~\cite{morris2015normology}.
%
The establishment of norms is rooted in shared social contexts, resulting in diverse cultural norms due to unique histories and cultural priorities~\cite{chiu2010intersubjective}.
%
In interpersonal communication, people rely on cultural norms to anticipate and interpret patterns of behavior. However, when observed behavior deviates from expected behavior, expectancy violations occur~\cite{burgoon1993interpersonal}.
%
Negative violations can lead to unfavorable outcomes, such as negative emotions and communication breakdowns, while positive violations can produce positive outcomes, such as an increase in perceived power~\cite{stamkou2019cultural, van2019dynamic}.
%
To detect and comprehend the consequences of norm violations, we employ Expectancy Violations Theory (EVT) which suggests that observers appraise expectancy violations with a valence (positive or negative) and intensity (high or low)~\cite{burgoon1993interpersonal}.
%
Mild-intensity violations may have a minimal effect, while more severe violations may cause significant consequences. This paper draws on EVT to develop a system capable of detecting norm violations, assessing their impact, and further rectifying them.

==> eacl2024-latex/6-limitation.tex <==
\section*{Limitations}
If needed.

==> eacl2024-latex/8-acknowledgement.tex <==
\section*{Acknowledgements}
If applied.
